ShapeFormer: Transformer-based Shape Completion via Sparse Representation

We present ShapeFormer, a transformer-based network that produces a distribution of object completions, conditioned on incomplete, and possibly noisy, point clouds. The resultant distribution can then be sampled to generate likely completions, each exhibiting plausible shape details while being faithful to the input. To facilitate the use of transformers for 3D, we introduce a compact 3D representation, vector quantized deep implicit function, that utilizes spatial sparsity to represent a close approximation of a 3D shape by a short sequence of discrete variables. Experiments demonstrate that ShapeFormer outperforms prior art for shape completion from ambiguous partial inputs in terms of both completion quality and diversity. We also show that our approach effectively handles a variety of shape types, incomplete patterns, and real-world scans.

==> fig/ablation_svq.tex <==
\begin{figure}[t!]
    \centering
    %\includegraphics[width=0.7\textwidth]{images/pipeline_svq.png}
    \includegraphics[width=\linewidth]{img/ablation_svq.pdf}
    \caption{The reconstruction quality of CSVQ with various resolutions.
    Given a dense complete point cloud (left column), our CSVQ can reconstruct high fidelity surface from it.
    And as the feature resolution increases the accuracy increases dramatically.
    Notice how the intricate details of the input are preserved at resolution 32 (CSVQ-32).
    And on resolution 16, our reconstruction results are already on par with state-of-the-art deep implicit method, ConvONet~\cite{Peng2020ConvONet}.
    The quantized features of CSVQ are visualized and shown in blue voxels and the different shades indicate different indices of the quantized feature.
    }
    \label{fig:ablation_svq} 
\end{figure}


==> fig/cmp_pointcloud.tex <==
\begin{figure}[h]
    \centering
    %\includegraphics[width=0.7\textwidth]{images/pipeline_svq.png}
    \includegraphics[width=\linewidth]{img/cmp_pointcloud.pdf}
    \caption{Visual comparison of our method with prior point cloud completion works (PCN~\cite{yuan2018pcn}, TopNet~\cite{Tchapmi2019topnet} and VRCNet~\cite{pan2021vrcnet}). Given a single view scan of an object as input (second column), our method can produce clean, smooth surface completions.
    Our highest probability completion (Ours) can reconstruct the missing parts with higher accuracy than prior works (third row).
    When the input is ambiguous (first row), among our predictions there still exists a completion that can accurately match the ground truth shape ($\text{Ours}_*$).
    }
    \label{fig:cmp_pointcloud} 
\end{figure}


==> fig/method_quantizer.tex <==
\begin{figure}[!t]
    \centering
    %\includegraphics[width=0.7\textwidth]{images/pipeline_svq.png}
    \includegraphics[width=\linewidth]{img/method_quantizer.pdf}
\caption{The workflow of the sparse quantizer. By removing the empty features from the feature grid, a sequence $\mathcal{S}_\mathbf{z}$ of positions and values of local features is obtained. Next, each feature value $\mathbf{z}_i$ is quantized to the nearest embedding $\mathbf{e}_{v_i}$ in a dictionary $\mathcal{D}$, and represented by the index $v_i$. The sequence of locations $c_i$ and dictionary indices $v_i$ together forms the sequence $\mathcal{S}$, which constitutes a lossily-compressed shape encoding.}
\label{fig:method_quantizer} 
\end{figure}


==> fig/overview.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=.99\columnwidth]{example-image-golden}
\hfill
\includegraphics[width=.99\columnwidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Outline -- }
A figure summarizing the entire algorithm
}
\label{fig:overview}
\end{figure*}

==> fig/pipeline_vqdif.tex <==
\begin{figure*}[!t]
    \centering
    %\includegraphics[width=0.7\textwidth]{images/pipeline_svq.png}
    \includegraphics[width=\textwidth]{img/pipeline_svq.pdf}
\caption{The architecture of Cloud SVQ. Given an input point cloud $\mathcal{P}$, the encoder compresses it to a sparse sequence $\mathcal{S}$. Then the decoder converts the sequence to a deep implicit function $f(\mathbf{x})$. By querying it with probes $x\in\mathcal{T}_\mathbf{x}$, the network predicts the occupancy grid $\mathcal{T}_{o}$ at resolution $128\times128\times128$, from which  mesh $\mathcal{M}$ is extracted via Marching Cubes algorithm. }
\label{fig:pipeline_svq} 
\end{figure*}

==> fig/results_failure.tex <==
\begin{figure}[h]
    \centering
    %\includegraphics[width=0.7\textwidth]{images/pipeline_svq.png}
    \includegraphics[width=\linewidth]{img/results_failure.pdf}
    \caption{An example of a shape completion failure case of ShapeFormer.
    The intricate details present in the input (second from left) are not preserved in the completions (gray shapes). The leftmost image shows the ground truth shape. }
    \label{fig:results_failure} 
\end{figure}


==> fig/results_progrecon.tex <==
\begin{figure}[h]
    \centering
    %\includegraphics[width=0.7\textwidth]{images/pipeline_svq.png}
    \includegraphics[width=\linewidth]{img/results_progrecon.pdf}
    \caption{Given an incomplete point cloud (in the left column), our method offers a number of possible completion (along the rows), where each is faithful to the input data and domain distribution. The vertical progression shows that the completions of our method converge to ground truth shape as the incompleteness diminishes.
    %\dc{this is a good example of a caption, XG, make the other captions as clear as this one.} \niloy{go from most partial to most complete scans}
    }

    \label{fig:results_progrecon} 
\end{figure}


==> fig/results_rotation.tex <==
\begin{figure}[h]
    \centering
    %\includegraphics[width=0.7\textwidth]{images/pipeline_svq.png}
    \includegraphics[width=\linewidth]{example-image-golden}
    \caption{Results on geometric transformation. \xgc{Placeholder.}}
    \label{fig:results_rotation} 
\end{figure}


==> sec/3_method_old.tex <==
\section{Cloud SVQ}

The goal of CSVQ is to learn a rich \textit{discrete} description for the local parts of the input point cloud, so that ShapeFormer can only focus on the global dependencies. 
On the other hand, it is also crucial that these local descriptions are compact due to the high complexity of transformer-based modeling of long-range dependencies.
Below, we demonstrate that a good balance between fidelity and non-local complexity can be achieved. 

As shown in Figure~\ref{fig:pipeline_svq}, CSVQ is an encoder-decoder architecture, where the encoder maps an input point cloud to a discrete sequence representation $\mathcal{S}$, while the decoder maps such a sequence to a deep implicit function $f(\mathbf{x})$.
The Sparse Quantizer, in the last stage of the encoder, plays a key role in learning the discrete description for the local parts, as described in Section~\ref{sec:quantizer}.

\subsection{Input and Output}

The input to CSVQ is a point cloud $\mathcal{P}\in\mathbb{R}^{N\times3}$ representing the dense sampling of a shape or its partial observation. 
During the training phase, we use complete dense clouds with $N>30000$ points in order to train CSVQ to capture local geometric details in the input.
At test time, CSVQ encodes a partial point cloud, which may be sparse or dense.
In Section~\ref{sec:results_realscan}, we demonstrate that even for sparse partial clouds obtained from real world scans, the sequence encoded by CSVQ still enables ShapeFormer to generate reasonable completions.

The output of the network is a deep implicit function $f(\mathbf{x})$ representing the occupancy field of a shape.
We query this function with a \emph{target point set} $\mathcal{T}_\mathbf{x}$.
By setting the target set to the coordinates of a grid of the desired resolution, we obtain the \emph{target occupancy field} of the shape, from which the surface mesh $\mathcal{M}$ is extracted using Marching Cubes.
At training time, the corresponding target occupancy $\mathcal{T}_o$ is known, and serves as the ground truth.

In the process, CSVQ learns to represent local shapes with a sparse sequence of 2-tuples $\mathcal{S}=\{(s_i, v_i)\}_{i=1}^K$, where $K$ indicates the number of local features. The sequence length $K$ is proportional to the shape's surface area. %\niloy{how do we estimate surface area?}

\subsection{Architecture}

\paragraph{Encoder}
The encoder first processes the input cloud with a local pooled PointNet~\cite{qi2017pointnet} to obtain a feature grid.
Similarly to prior work \cite{Peng2020ConvONet}, the local pooled PointNet aggregates features within a grid cell in contrast to the original PointNet, where all point features are pooled together to obtain a global feature. Specifically, we use a grid of resolution $64$ with feature size of $32$.

Next, in order to reduce the number of local features, the high resolution feature grid is downsampled to a lower resolution one, using several consecutive strided convolutions blocks.
The parameters of these blocks are carefully set to have the least receptive field, since a large receptive field lets each grid feature cover a larger region, reducing the sparsity of the representation. 
See the supplementary material for details. %\niloy{make sure this is included in supl.}
The down-sampled resolution $\mathit{R}$ balances between fidelity and representation size. We empirically found that $\mathit{R}=16$ best suites our shape completion task. See Section~\ref{sec:ablation_svq} for the effect of various resolutions.

Due to their limited receptive field, the down-sampled grid features only perceive local regions of the input cloud. Since the cloud only resides in a small portion of the 3D volume, many of these features encode no geometry at all. 
The last encoder module, the \textit{Sparse Quantizer}, records the grid location of only the non-empty local features, and discretizes their continuous values using Vector Quantization \cite{van2017vqvae1} (see Section~\ref{sec:quantizer} for details). Thus, a sparse discrete sequence representation is obtained.


\paragraph{Decoder}
The decoder consists of three components: a 3D U-Net \cite{cciccek2016unet3d}, an upsampler, and an implicit decoder. It first projects the quantized sparse sequence back to a 3D feature grid, which serves as the input for the 3D U-Net.

In contrast to the encoder, the decoder is designed to have a large receptive field. 
This is because in order for the implicit decoder to infer whether a probe lies inside or outside of the shape, we need global knowledge. This is in alignment with prior works \cite{Peng2020ConvONet, Erler2020Points2Surf}.
More specifically, we use a 3-step U-Net to increase the receptive field, which integrates both local and global information.

The upsampler has the same number of scaling stages as the down-sampler but it has a larger receptive field by design.
Lastly, similarly to prior work \cite{Peng2020ConvONet}, the implicit decoder consists of multiple ResNet blocks.
It takes querying probe points $\mathcal{T}_\mathbf{x}$ and predicts their occupancy probability $\mathcal{T}_{o}$.


\subsection{Sparse vector quantization} \label{sec:quantizer}
\input{figures/method_quantizer}
%\input{figures/svq_show}vocabular

As illustrated in Figure~\ref{fig:method_quantizer}, given the 3D grid of local geometric features as input, the Sparse Quantizer first removes the empty features to obtain a sparse sequence of local features, namely
\begin{equation}
    \mathcal{S}_\mathbf{z} = \{(c_i, \mathbf{z}_i)\}_{i=0}^{K-1},
\end{equation}
where $c_i$ indicates the $i$-th raveled 3D index of a grid cell, $\mathbf{z}_i$ denotes the local geometric feature therein, and $K$ is the number of non-empty features.

In order to efficiently represent the spatial location, we unroll the 3D coordinate to a single index, since we only operate at a grid that is at most 32 resolution, each index will be at most just a 15-bit integer so we do not encounter the problem as in prior works \cite{sun2020pointgrow, nash2020polygen}.
%in the following way: $c=x + \text{res}\cdot( y + \text{res}\cdot z )$, here $\text{res}$ indicates the resolution of the grid, and $x,y,z$ are the three indices of that grid.
%The value of the raveled coordinate $c$ has a discrete choice from $\text{res}^3$ choices. While this would lead to too many choices for raw points generation (where $\text{res}=256$) \cite{sun2020pointgrow, nash2020polygen}, we do not have the same problem since we only model voxel grid coordinates (e.g., $\text{res}\leq 32$).
%\dlc{I have to insist again, that this is way too basic to describe in such detail. Everyone knows how to flatten a multi-dimensional array. We can just say that since the grid is at most 32 resolution, each index is just a a 16-bit integer.}
%
Also, we mark the empty feature $\mathbf{z}_\varnothing$ and later utilize it as the filling feature for projecting the sparse sequence back to feature grid again for decoding.
%\dlc{Not clear; how/where do you save it?}
%\xgc{We pick an "empty" grid cell and set it as $\mathbf{z}_\varnothing$, then it is considered as an another output along with the sequence. Then given the empty feature along with the sequence, our decoder can project them back to dense feature grid. So the actual representation is empty feature + sequence.}

Following the idea of neural discrete representation learning \cite{van2017vqvae1}, the features of sequence $\mathcal{S}_\mathbf{z}$ are quantized by clamping it to the corresponding nearest entries in a dictionary $\mathcal{D}$ of embeddings $\{\mathbf{e}_j\}_{j=0}^{V}$ and we save the indices of these embeddings as,
\begin{equation}
    v_i = \text{argmin}_{j\in[0,V)} \|\mathbf{z}_i-\mathbf{e}_j\|,
\end{equation}
where $V$ is the vocabulary size of the dictionary $\mathcal{D}$.

This can be viewed as a process of lossy compression, where much of the statistical redundancies in the local features are eliminated without loosing much representation power. %\dlc{Do we really need to explain this?} 
%In Section~\ref{sec:ablation_svq} we evaluate how quantization affects reconstruction accuracy. 
%\dlc{Is there indeed going to be such an evaluation?}

Thus, starting from an input point cloud, we get a sequence of discrete 2-tuples 
\begin{equation}
    \mathcal{S}=\{(c_i, v_i)\}_{i=0}^{K-1}
\end{equation}
for consumption by the ShapeFormer, as introduced later. 

% sequence before quantization: \mathcal{S}_z = {(c_i, \mathbf{z}_i)}_{i=0}^K
% sequence after  quantization: \mathcal{S}   = {(c_i, v_i)}_{i=0}^K
% codebook and embeddings: \mathcal{Z} = {\mathbf{e}_v}_{v=0}^{V-1}


%8 or 16 or 32, resolution effect \ref{sec:vq_resolution} % *3
%size of sparse voxel (sequence length) \ref{fig:svq_show}


\subsection{Training and inference}

%After the output of the network is obtained, that is, the deep implicit function $f(\mathbf{x})$ and the sequence representation $\mathcal{S}$, our devised training loss guides the network to improve the reconstruction accuracy.
The training loss for CSVQ is composed of two terms: reconstruction loss and commitment loss \cite{van2017vqvae1}:
\begin{equation}
    \mathcal{L}_\text{svq} = \mathcal{L}_\text{rec} + \beta  \mathcal{L}_\text{commit},
    %L_{vq}
\end{equation}
where $\beta$ is a balancing factor, set to $\beta=0.01$ in our experiments.

The reconstruction loss forces the network to correctly classify whether a target point lies inside or outside of the shape. 
%\xgc{
%I think the goal of this term is to confine the features within certain range, which makes the quantization easier. I have tested to remove this term, which indeed hurts the quality of the results.
%Quote from the original VQVAE paper\shortcite{van2017vqvae1}: \textit{To make sure the encoder commits to an embedding and its output does not grow, we add a commitment loss}}
% 
Specifically, we define the reconstruction loss as, 
\begin{equation}
    \mathcal{L}_\text{rec} = \frac{1}{T}\sum_{i=0}^{T-1}\text{BCE}\large( f(\mathbf{x}_i), o_i \large),
\end{equation}
where BCE stands for the binary cross entropy loss and $\mathbf{x}_i$ and $o_i$ are the target point and its occupancy value, respectively, and $T$ is the size of the target set.
%
During training, we select the target set $\mathcal{T}_x=\{\mathbf{x}_{i=0}^{T-1}\}$ and its occupancy value $\mathcal{T}_o=\{o_{i=0}^{T-1}\}$ in a similar fashion to Chibane et al.~\shortcite{chibane20ifnet}, that is, randomly selecting two groups of points on the shape surface and adding a random Gaussian shift with two different scales.

The commitment loss forces the local features to stay close to their nearest embeddings in the dictionary, thus keeping the range of the embeddings bounded. We define the loss as, 
\begin{equation}
    \mathcal{L}_\text{commit} = \frac{1}{K}\sum_{i=0}^{K-1}(\mathbf{z}_i-\text{sg}[\mathbf{e}_{v_i}])^2, %L_{vq}
\end{equation}
where $\mathbf{z}_i$ is the continuous feature before clamping it to $\mathbf{e}_{v_i}$ and sg stands for stop gradient operator which prevents the embedding from being updated during optimization.

We do not use explicit loss to update dictionary embeddings like in the original VQVAE \cite{van2017vqvae1}. Instead, we use the alternative exponential moving average (ema) to update the embeddings, see the appendix of the original paper for more details.

At inference time, we set the target set as the regular grid sampling of resolution 128 to enable high-quality surface reconstruction.


\section{ShapeFormer}
\input{figures/pipeline_shapeformer}
%\input{figures/method_nextcond}
% \xgc{moved to supp}
Given the sequence encoding of a partial point cloud $\mathcal{S}_\mathcal{P}$, the goal of ShapeFormer is to learn the conditional joint distribution $p(\mathcal{S}_\mathcal{C}|\mathcal{S}_\mathcal{P})$, where $\mathcal{S}_\mathcal{C}$ is a sequence encoding of a possible complete shape.
Once the conditional distribution is modeled, we are able to obtain different shape completions $\mathcal{S}_\mathcal{C}$ by sampling the distribution for the same $\mathcal{S}_\mathcal{P}$. This effectively turns the shape completion problem into a sequence generation one.

Ideally, the partial sequence is a strict sub-sequence of the complete one, in which case one can utilize a masked language model such as BERT~\cite{devlin2018bert} to model the above distribution.
This strategy has been proved effective for image completion~\cite{wan2021ict}.
However, in our case, $\mathcal{S}_\mathcal{P}$ is not necessarily contained in $\mathcal{S}_\mathcal{C}$ due to noise and sparsity of the point cloud, which means we need to not only predict the missing elements in $\mathcal{S}_\mathcal{C}$, but also need to update (i.e., denoise) the elements observed in $\mathcal{S}_\mathcal{P}$.
Hence, we adopt an alternative auto-regressive objective for language model by modeling the above distribution, conditioned on the partial observation $\mathcal{S}_\mathcal{P}$, to generate complete sequences $\mathcal{S}_\mathcal{C}$.
%\dlc{Not clear, you just said we may need to update the elements of Sp and not just complete it.}
This strategy has been shown successful in the task of conditional image synthesis \cite{esser2020taming}.

We model this distribution by factoring it using the probability chain rule and separately modeling the individual distribution of each element conditioned on its previous elements.
Since our sequences consist of 2-tuples, we also factor out the joint distribution of the tuples as $p(c_i,v_i)=p(c_i)  p(v_i | c_i)$ (see also \cite{nash2021DCTransformer, dieleman2021SlowAEs, wang2020sceneformer}).
More specifically, we use ShapeFormer to separately model the distribution of each element by:
\begin{align*} 
p_{c_i} &= p(c_i|\mathbf{c}_{   < i}, \mathbf{v}_{<i}, \mathcal{S}_\mathcal{P}; \theta) \\ 
p_{v_i} &= p(v_i|\mathbf{c}_{\leq i}, \mathbf{v}_{<i}, \mathcal{S}_\mathcal{P}; \theta),
\end{align*}
where $\theta$ indicates model parameters, and $p_{c_i}$ and $p_{v_i}$ are the distributions of the coordinate and the index value of the $i$-th element of $\mathcal{S}_\mathcal{C}$, conditioned on previously generated elements and the parital sequence $\mathcal{S}_\mathcal{P}$. Note that $p_{v_i}$ is also conditioned on its own coordinate $c_i$, and not only on the previous 2-tuples.
%
Thus, we model the distribution of the sequence as:
\begin{equation}
    p(\mathcal{S}_\mathcal{C}|\mathcal{S}_\mathcal{P}) = 
            \prod_{i=0}^{K-1}   p_{c_i}\cdot p_{v_i},
\end{equation}
where $K$ is the length of the complete sequence $\mathcal{S}_\mathcal{C}$.


\subsection{Input and output} \label{sec:shapeformer_input}

During training, the input to the ShapeFormer consists of the concatenated sequence of $\mathcal{S}_\mathcal{P}$ and $\mathcal{S}_\mathcal{C}$, as shown in Figure~\ref{fig:pipeline_shapeformer}.
Since these sequences both have variable lengths, we append an end-token ([END]) to each sequence to indicates when the sequence terminates. 

We find that model convergence may be accelerated by adding an extra input embedding derived from the coordinate indices; see the supplementary material for more details.

%In addition to the 2-tuples, we compute a special extra sequence of next greater coordinate in parital sequence to help ShapeFormer find the correspondence between the two sequences. 
%\dlc{Sorry, completely unclear...}
%We find adding this sequence will accelerate convergence for model training (See Section \ref{sec:ablation_embeddings}).
%As illustrated in Figure~\ref{fig:method_nextcond}, for the $i$-th element in $\mathcal{S}_\mathcal{C}$ %\dl{$\mathcal{S}_\mathcal{S}$?} 
%we assign an $n_i$ which is the next greater coordinate in the partial sequence according to its coordinate $c_i$.
%And for $\mathcal{S}_\mathcal{P}$, we set its $n_i$ as same as its coordinate $c_i$.

%Although the sequential position no longer directly encode spatial location, it can still encode the relative positions between sequence elements which helps ShapeFormer to better understand their relations.

Next, as in prior works \cite{nash2021DCTransformer, dieleman2021SlowAEs}, all these indices are turned into learnable embeddings and are additively combined as the input embedding for ShapeFormer.


%Unlike prior work \cite{esser2020taming}, both parital and complete sequence has variable length in our case.
%So instead of resuming the sequence position after partial sequence end, we restart the positioning by using separate positional embeddings for partial and complete sequence. \dlc{not clear, but perhaps this is again too low level, and perhaps should be described in appendix/supplementary or not at all.}

The outputs of the ShapeFormer are the predicted categorical conditional distributions for each of the sequence elements: $\{(p_{c_i}, p_{v_i})\}_{i=1}^K$. Note that this essentially shifts the complete sequence to the right by one element. 
%, see Figure~\ref{fig:pipeline_shapeformer}.
%\dlc{referring to the detailed diagram only at the end is pointless... refer and make use of it from the start.}
% ablation: w/o positional encoding, separate vs continuous positional encoding
% The input to ShapeFormer are the 2-tuples sequences of partial sequence and complete sequence.
% In order for ShapeFormer to better learn the sequences, we append a special \textit{end token} for both partial and complete sequence
% The output is the categorical conditional probability distribution for each element of the sequence
% \begin{equation}
%   \{(p(c_i|c_{<i}, v_{<i}, \mathcal{S}_\mathcal{P}), p(c_i|c_{\leq i}, v_{<i}, \mathcal{S}_\mathcal{P})) \}_{i=0}^{K-1}
% \end{equation}
% ${ }$

\subsection{Architecture}
Different approaches have been applied to build a transformer model that can predict tuple sequences. 
One direct solution is to flatten the tuple sequence \cite{sun2020pointgrow}, which has the disadvantage of doubling the sequence length.
Another popular option is to stack multiple transformers, where each predicts one tuple item \cite{wang2020sceneformer, nash2021DCTransformer, dieleman2021SlowAEs}.
We also use two stacked transformers that to process 2-tuples in a single pass, as shown in Figure~\ref{fig:pipeline_shapeformer}.

The main components of ShapeFormer are two causally-masked transformers, which consist of multiple decoder-only transformer blocks \cite{radford2019GPT2}. 
The first transformer learns to predict the coordinate of the next tuple, conditioned on previous tuples; while
the second one learns to predict the value of the next element conditioned on previous tuples and the (predicted) coordinate index of next element. Thus, the output feature of the first transformer is additively mixed with the input embedding of the second transformer.

Each transformer is followed by an output head, which converts the feature produced by the transformer into a categorical distribution of the next sequence element.
Both output heads consist of two fully connected layers, followed by a softmax layer.


%\xgc{How DCTransformer described their architecture: (see comments in latex source code)}
% In order to model the three distinct variable types in DCT
% coordinate lists, our architecture must yield autoregressive
% predictions for each variable, and should condition on all
% the available context. One possible approach is to flatten
% the tuples, and to pass the resulting values through a single
% Transformer decoder, projecting the resulting states to logits
% as appropriate for each variable. To increase the amount of
% content modelled in a particular target sequence, we instead
% opt to use three distinct Transformer decoders, one for each
% of the channel, position and value predictions. The three decoders are stacked on top of one another, yielding sequence
% lengths three times smaller than flattened sequences.
%\xgc{And SlowAE's description: (in comments)}

% The main component is a causally masked Transformer with relative position self-attention, which contains
% the bulk of the learnable parameters. The input consists of
% a set of learnable embeddings which are additively combined...

% Empirically, we find that it suffices to stack a two-layer multi-layer perceptron
% (MLP) on top of the Transformer and feed it an embedding
% of vn+1 as a side-input to predict ln+1. As a result, we
% do not need to flatten the (value, length)-tuples into an
% alternating sequence. This is significant, as the cost of the
% attention mechanisms inside the Transformer is quadratic
% in the sequence length. Architecture and training details are
% provided in appendix


\subsection{Training and sampling}
The training objective of ShapeFormer is to minimize the negative log-likelihood of the complete sequence, conditioned on the given partial sequence.
At the element-wise level, the objective is reduced to multi-class classification.

After the model is trained, ShapeFormer performs shape completion by sequentially sampling the next element of the complete sequence until an end token ([END]) is encountered. Given the partial sequence, we alternatively sample the new coordinate and value index using nucleus sampling \cite{holtzman2019nucleus}, where only the few top choices, for which the sum of probabilities exceeds a threshold $p_n$, are kept and the remaining probability mass are redistributed across them. %nucleus sampling, p=.4

%\xg{
%Add discussion on probability
%}

Also, in order to ensure that the sampled coordinate sequence is monotonic, we mask out those coordinate choices that are smaller or equal to the current maximum coordinate.
This only redistributes the probability mass toward valid choices and has no negative effect on model performance. 
%More specifically, at each sampling step for coordinate, we mask out the coordinate choices that are smaller or equal to the current maximum coordinate. 
%so that the coordinate sequence are guaranteed to be monotonically increasing.

%The rule for masking can be found at the supplementary material.




==> sec/X_instructions.tex <==
% --- repeat the title (AT: haven't found a more elegant way to do this...)
\twocolumn[
\centering
\Large
\textbf{\LaTeX\ Author Guidelines for \confName~Proceedings (2022)}
\vspace{1.0em}
] %< twocolumn
\appendix

\setcounter{section}{0}
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/old_introduction.tex <==
\section{Introduction}
\label{sec:intro}
\input{fig/teaser}
Shapes are typically acquired with cameras that probe and sample surfaces. They rely on line of sight and, at best, can obtain information for visible parts of objects. Hence, sampling complex real-world geometry is inevitably imperfect, resulting in varying sampling density and missing parts. This problem of surface completion has been extensively investigated in the last decades \cite{berger2017survey}. The central challenge is to compensate for incomplete data by inspecting non-local hints in the observed data to infer missing parts using various forms of priors. 
%\xgc{Maybe mention other sources for partial shape? such as "incomplete work in the user modeling interface"(part-level incomplete)}

%Since surface completion is inherently an ill-posed problem, which suggests various sensible compilation to the missing part.

%global&local deep priors (DIF)
In the context of data priors, \xg{deep implicit functions (DIF) have recently emerged as an effective  representation for learning high-quality surface completion. To distill shape priors from data, earlier works in this family \cite{zhiqin2019imnet, lars2019occnet, park2019deepsdf} encode each shape using a single latent vector.
However, such \textit{global} coding, due to their lack of spatial structure, usually lead to completions that do not respect toward the parital observation.
Combining global code with latent codes of local regions, local approaches \cite{Erler2020Points2Surf, Peng2020ConvONet, chibane20ifnet, jiang2020lig, genova2020ldif, chen2021mdif} can faithfully preserve geometric details of the input in the completion.
However, for \textit{ambiguous} input, that is, when there are multiple complete shapes corresponding to the input such as the examples shown in Figure.~\ref{fig:teaser}, current local DIF methods, due to their deterministic nature, usually fail to produce meaningful shapes in unseen regions.
One possible solution is to combine generative models to handle the input uncertainty.
However, for representations that contain huge statistical redundancy, as in the case of current local methods, such combination is infeasible, or at least limited \cite{sun2020pointgrow}, since they will excessively allocate model capacity towards perceptually irrelevant details \cite{Fauw2019HierarchicalAR, dieleman2021SlowAEs}

%Instead of learning global shape priors, an alternate option is to use \textit{local} priors (e.g., local implicits), which significantly improves generalization and can faithfully represent local geometric details.
% generative completion
% Need generative models (GM)
% GM needs good repr.
% either too compressed, easy learning + no structure
% or too heavy, hard learning + good structure
% On the other hand, conditional generative models are suited for modeling such input uncertainty.
% A good 3D representation is crucial for applying such models to shape completion. It should be both spatially structured and compact. 
% A structured representation enables the model to produce completions that preserve the input. 
% And in contrast with a raw representation, a compact one, which captures salient features and is small in size, makes the distribution modeling more efficient and effective \cite{dieleman2021SlowAEs, Fauw2019HierarchicalAR}.
% Existing generative approaches for point cloud completion either using a compact but unstructured representation \cite{wu2020cGAN}, which produces completions misaligned with input, or directly using raw point cloud \cite{zhou2021pvd}, which is only effective for completing simple shapes with limited number of points.
%naively deploying transformers on point sets is infeasible, or at least limited \cite{nash2020polygen, sun2020pointgrow, zhou2021pvd}
%Applying generative models directly to raw data usually results in excessive allocation of model capacity towards perceptually irrelevant details \cite{Fauw2019HierarchicalAR, dieleman2021SlowAEs},

% VQ
A promising alternative is to compress the local codes to a sequence of discrete, vector quantized features, which greatly reduces the representation size while keeping the structure. Applying transformer-based generative models toward such sequences of discrete variables have been shown effective for image generative pre-training \cite{chen2020imagegpt, bao2021beit} and various image synthesis tasks \cite{razavi2019vqvae2,chen2020imagegpt,esser2020taming} including pluralistic image completion \cite{wan2021ict}.
Unfortunately, directly deploying such strategy for 3D shape will lead to a sequence length of cubic feature resolution. Due to the transformer's own quadratic complexity on sequence length, only very coarse feature resolution is feasible in this case, which can barely represent meaningful shapes. 
Besides, unlike image completion \cite{wan2021ict} where the model only need to predict for unseen regions (The BERT \cite{devlin2018bert,bao2021beit} strategy), for 3D shape completion, the input features could also come from incomplete observations and keeping them unchanged will lead to incomplete results.
}
% A promising alternative is to use transformer-based autoregressive models that have been shown to effectively learn such distributions for discrete variables \cite{vaswani2017transformer}.
% Unfortunately, naively deploying transformers on point sets is infeasible, or at least limited, since transformers have a quadratic complexity in the input sequence length~\cite{nash2020polygen,sun2020pointgrow}. 
% One solution is to represent shapes using local quantized features, and apply transformers to learn their long-range dependencies. This, however, requires an efficient local discrete representation that achieves good balance between feature locality and expressiveness. 

\xg{
In this paper, we introduce Vector Quantized Deep Implicit Functions (\textit{VQDIF}), a novel 3D representation which is both compact and structured, that can represent complex 3D shapes with decent accuracy while being rather small in size.
The core idea is to sparsely encode shapes as sequences of discrete 2-tuples, each representing both the position and content of a non-empty local feature. 
These sequences can be decoded to deep implicit functions from which high quality surfaces can subsequently be extracted.
Due to the sparse nature of 3D shapes, such encoding reduces the sequence length from cubic to quadratic toward feature resolution, thus enables effective combination with generative models.
%We specifically control the receptive field of the encoder to encourage sparsity, leading to shorter sequence, which 

We also design \textit{ShapeFormer}, a transformer-based autoregressive model for VQDIF, which solves shape completion by generating the sequence for complete shapes conditioned on the sequence for partial observation.
The ShapeFormer is trained to sequentially predicting the conditional distribution of both location and content over the next element.
Unlike BERT-based methods \cite{wan2021ict, devlin2018bert, bao2021beit}, in order to generate complete sequence from scratch while according to the partial one, we simply prepend the partial sequence to the complete one during autoregressive training and sampling. This strategy has been proved effective for conditional synthesis for both texts \cite{liu2018wikigen} and images \cite{esser2020taming}.

We demonstrate the ability of ShapeFormer to produce diverse high-quality completions for ambiguous partial observation for various shape types, including CAD models and human body; for various incomplete sources such as scans and missing parts. Figure~\ref{fig:teaser} shows several such examples. We further show that our approach can be readily applied to real world scans.
%Experiments demonstrate our method outperforms prior arts for shape completion from ambiguous partial input in terms of both completion quality and diversity.

In summary, our contributions include:
%\paragraph{Contributions}
\begin{itemize}[leftmargin=*]
\setlength\itemsep{-.3em}
\item a novel DIF representation based on sequence of discrete variables that can represent 3D shapes in decent accuracy with a rather small size;

\item a transformer-based autoregressive model based on the new representation that predicts multiple high-quality completed shapes conditioned on the partial input;

\item state-of-the-art results for multi-modal shape completion in terms of completion quality and diversity. The FPD score on PartNet is improved by at most 1.7 compared with prior multi-modal method cGAN~\cite{wu2020cGAN}.

\end{itemize}
}

==> tab/ablations.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Ours v0 & Frumpy \\
Ours v1 & Frobbly \\
\textbf{Ours} & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} %< \resizebox
\caption{
% 
\textbf{Ablations} -- our decisions are well justified.
% 
} % \caption
\label{tab:ablations}
\end{table}

==> tab/sota.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} % \resizebox
\caption{
% 
\textbf{State of the art} -- Glory to the bold numbers.
% 
} % \caption
\label{tab:sota}
\end{table}

==> tab/table_ablation_svq.tex <==
\begin{table}[t!]%
	\label{tab:ablation_csvq}
	\begin{minipage}{\columnwidth}
		\begin{center}
		%	\begin{tabular}{p{2.4cm}|r|r|r|r}
		\begin{tabular}{r||r|r|r|r} 
		    \toprule
    	    \textbf{Metric}             & ConvONet  & CSVQ-8    & CSVQ-16   & CSVQ-32   \\ 
		    \midrule
    		 CD$\times10^{-3}$          & 0.81      & 1.21      & 0.83      & 0.61    \\ 
    		 Seq. length                & 32768     & 66        & 245       & 623     \\ 
		    \bottomrule
		\end{tabular}
		\end{center}
	\end{minipage}
	\caption{
	Our CSVQ can balance between reconstruction accuracy and sequence length.
	We evaluate previous state-of-the-art deep implicit method ConvONet~\cite{Peng2020ConvONet} and our CSVQ in three different resolutions: CSVQ-8, CSVQ-16 and CSVQ-32.
	We measure the performance with Chamfer Distance (CD) and sequence length averaging across all shapes.
	}
\end{table}%

% \begin{table}[t!]%
% 	\caption{
% 	Our CSVQ can balance between quality and sequence length.}
% 	\label{tab:ablation_csvq}
% 	\begin{minipage}{\columnwidth}
% 		\begin{center}
% 		%	\begin{tabular}{p{2.4cm}|r|r|r|r}
% 		\begin{tabular}{l||l|l|l}
%     		\hline
%     	    \textbf{Method}             & CD           & Avg. length       \\ \hline
%     		 ConvONet                   & 0.81         & 32768         \\ \hline
%     		 CSVQ-8                     & 2.21         & 94          \\ \hline
%     		 CSVQ-16                    & 0.86         & 316         \\ \hline
%     		 CSVQ-32                    & 0.61         & 942         \\ \hline
% 		\end{tabular}
% 		\end{center}
% 	\end{minipage}
% \end{table}%


==> tab/table_realscan.tex <==
\begin{table}[t!]%
	\caption{
	Comparison with prior works on real scans.}
	\label{tab:cmp_realscan}
	\begin{minipage}{\columnwidth}
		\begin{center}
		%	\begin{tabular}{p{2.4cm}|r|r|r|r}
		\begin{tabular}{l||l|l|l|l|l}
    		\hline
    		                            & \multicolumn{2}{|c|}{ScanNet} 
    		                            & \multicolumn{2}{|c|}{MatterPort3D} 
    		                            & KITTI \\ \hline
    	    \textbf{Method}             & Chair  & Table  & Chair  & Table  & Car \\ \hline
    		 pcl2pcl                    & -      & -      & -      & -      & -   \\ \hline
    		 cGAN                        & -      & -      & -      & -      & -   \\ \hline
    		 ShapeInversion             & -      & -      & -      & -      & -   \\ \hline
    		 \textbf{$\text{Ours}$}     & -      & -      & -      & -      & -   \\ \hline
		\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%

